Reinforcement Learning With Reward Machines in Stochastic Games

We investigate multi-agent reinforcement learning for stochastic games with complex tasks, where the reward functions are non-Markovian. We utilize reward machines to incorporate high-level knowledge of complex tasks. We develop an algorithm called Q-learning with reward machines for stochastic games (QRM-SG), to learn the best-response strategy at Nash equilibrium for each agent. In QRM-SG, we define the Q-function at a Nash equilibrium in augmented state space. The augmented state space integrates the state of the stochastic game and the state of reward machines. Each agent learns the Q-functions of all agents in the system. We prove that Q-functions learned in QRM-SG converge to the Q-functions at a Nash equilibrium if the stage game at each time step during learning has a global optimum point or a saddle point, and the agents update Q-functions based on the best-response strategy at this point. We use the Lemke-Howson method to derive the best-response strategy given current Q-functions. The three case studies show that QRM-SG can learn the best-response strategies effectively. QRM-SG learns the best-response strategies after around 7500 episodes in Case Study I, 1000 episodes in Case Study II, and 1500 episodes in Case Study III, while baseline methods such as Nash Q-learning and MADDPG fail to converge to the Nash equilibrium in all three case studies.

==> alternative_example.tex <==
!TEX root = main.tex

% \color{orange!90!black}

\subsection{Alternative Motivating Example}

As a motivating example, let us consider an autonomous vehicle whose task is to navigate in a residential area, as sketched in Figure~\ref{fig:ex:road-map}.
As common in many European countries, some of the streets are priority streets.
While traveling on a priority street, a car has the right-of-way and does not need to yield to traffic on intersections.
Typically, priority roads start with a special sign and ends with a special sign. 
(In reality, there might be different signs or conditions for an end of a priority road, but in this simple example we are abstracting that away.)
In the example of Figure~\ref{fig:ex:road-map}, both roads going from west to east are priority roads (indicated by a gray shading), whereas the roads going from north to south are ordinary roads.

\begin{figure}[th]
	\centering
	\begin{tikzpicture}
		% Road
		\draw[double=white, double distance=5mm, line width=.5mm] (0, 0) -- (6, 0) (0, -2) -- (6, -2) (2, 1) -- (2, -3) (4, 1) -- (4, -3);
		\fill[gray!25] ([yshift=-2.5mm]0, 0) rectangle ([yshift=2.5mm]6, 0) ([yshift=-2.5mm]0, -2) rectangle ([yshift=2.5mm]6, -2);
		
		% Markings
		\draw[dashed] (0, 0) -- (6, 0) (0, -2) -- (6, -2);
		\draw[dashed] (2, 1) -- (2, .25) (4, 1) -- (4, .25) (2, -.25) -- (2, -1.75) (4, -.25) -- (4, -1.75) (2, -2.25) -- (2, -3) (4, -2.25) -- (4, -3);
	
		% Labels
		\node[font=\bfseries] at (-.5, 0) {A};
		\node[font=\bfseries] at (6.5, -2) {B};
	
	\end{tikzpicture}
	
	\caption{Map of a residential area} \label{fig:ex:road-map}
\end{figure}


\begin{figure}[b]
		\centering                              
		\includegraphics[width=9cm]{figures/traffic.pdf}                                         
		\caption{\ZX{Map of a residential area}} \label{fig:ex:road-map}
	\end{figure}   

Let us assume that the task of the autonomous vehicle is to drive from position ``A'' (a start position) on the map to position ``B'' while obeying the traffic rules.
To simplify matters, we are here only interested in the traffic rules concerning the right-of-way and how the vehicle acts at intersections.
Moreover, we make the following two further simplifications: (1) we assume that the vehicle correctly senses the beginning and the end of a priority road (by recognizing the corresponding signs) and (2) we are only interested in whether or not the vehicle should yield to vehicles coming from the intersecting road (in a realistic scenario, the turning vehicle clearly also needs to consider opposing traffic).
%other vehicles on its right side 

Even for this simplified view, a memory-less policy does not suffice as the optimal action at any intersection depends on whether or not the vehicle is traveling on a priority road (which it might have entered multiple intersections before).
More precisely, in our model, the vehicle is obeying the rules if and only if
\begin{itemize}
	\item it is traveling on a normal road, has traffic on the intersecting road, and yields to the traffic;
	\item it is traveling on a normal road, has no traffic on the intersecting road, and does not yield; or
	\item it is traveling on a priority road and does not yield (regardless of whether there is traffic on the intersecting road).
\end{itemize}
In particular, the vehicle violates the rules and does not get a reward if it yields on a priority road or on a normal road when there is no traffic on the intersecting road.

An example reward machine for traveling on priority roads is shown in Figure~\ref{fig:ex:reward-machine}.
Intuitively, state $p_0$ corresponds to the vehicle traveling on a normal road, while $p_1$ corresponds to the vehicle traveling on a priority road.
While in $p_0$, the vehicle ends up in a sink state $p_x$ in case there is a traffic ($\mathit{tr}$) and it does not yield ($\lnot \mathit{y}$), or in case there is no traffic ($\lnot \mathit{tr}$) and it does yield ($\mathit{y}$). %; in both cases, the reward machine remains in state $p_0$.
While in state $p_1$, on the other hand, the vehicle gets to the sink state if it yields, regardless of whether there is traffic on the right.
The reward machine switches between states $p_0$ and $p_1$ on entering and exiting a priority road (indicated by $\mathit{pr}$ and $\lnot \mathit{pr}$, respectively).
Finally, the reward 1 is obtained if from either $p_0$ or $p_1$ place $B$ is reached.


\begin{figure}[th]
	\centering
	\begin{tikzpicture}
		\node[state] (0) at (0, 0) {$p_0$};
		\node[state] (1) at (3.5, 0) {$p_1$};
		\node[state] (x) at (0, - 3.5) {$p_x$};
		\node[state] (2) at (4.5, - 3.5) {$p_2$};
		\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
		\draw[->] (0) to[bend right] node[sloped, below, align=center] {$(\lnot B \land \mathit{tr} \land \lnot y, 0)$ \\ $(\lnot B \land \lnot \mathit{tr} \land y$,0)} (x);
		\draw[->] (0) to[loop above] node[align=center] {$(\lnot B \land \lnot\textit{pr}, 0)$\\$(\lnot B \land \textit{tr} \land \mathit{y}, 0)$ \\ $(\lnot B \land \lnot\textit{tr} \land \lnot\mathit{y}, 0)$} ();
		\draw[->] (0) to[bend right=10] node[sloped, above, align=center] {$(B, 1)$} (2);
		\draw[->] (0) to[bend left=20] node {$(\lnot B \land \mathit{pr}, 0)$} (1);			
		\draw[->] (1) to[loop above] node[align=center] {$(\lnot B \land \lnot\mathit{y}, 0)$ \\ $(\lnot B \land\mathit{pr}, 0)$} ();
		\draw[->] (1) to[bend left] node [above]{$(\lnot B \land\lnot\mathit{pr}, 0)$} (0);
		\draw[->] (1) to[bend left=20] node[align=left, sloped, below] {$(y,0)$} (x);
		\draw[->] (1) to[bend left=10] node[align=center, sloped] {$(B, 1)$} (2);
		\draw[->] (x) to[loop below] node {$(*,0)$} ();
		\draw[->] (2) to[loop below] node {$(*,0)$} ();
	\end{tikzpicture}	
	\caption{Reward machine for traveling on priority roads} \label{fig:ex:reward-machine}
\end{figure}


\begin{figure}[th]
	\centering
	\begin{tikzpicture}
	\node[state] (0) at (-0.5, 0) {$p_0$};
	\node[state] (1) at (4.5, 0) {$p_1$};
	\node[state] (2) at (4.5, 4.5) {$p_2$};
	\node[state] (3) at (0, - 3.5) {$p_3$};
	\node[state, accepting] (4) at (7, - 3.5) {$p_4$};
	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
	\draw[->] (0) to[left] node[above, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (1);
	\draw[->] (0) to[loop above] node[align=center] {$(\lnot s \land \mathit{pr}, 0)$} ();
	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(s \land \lnot\mathit{pr}, 0)$} (2);
	\draw[->] (2) to[bend right] node[sloped, below, align=center] {$(\lnot s \land \mathit{pr}, 0)$} (0);
	\draw[->] (2) to[bend right] node[below, align=center] {$(s \land \lnot\mathit{pr}, 0)$} (3);
	\draw[->] (0) to[bend right] node[below, align=center] {$(s \land \mathit{pr}, 0)$} (3);
	\draw[->] (1) to[bend right] node[below, align=center] {$(\lnot s \land \mathit{pr}, 0)$} (3);
	\draw[->] (1) to[bend left] node[above, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (3);
	\draw[->] (0) to[bend right] node[below, align=center] {$(B, 1)$} (4);
	\draw[->] (1) to[bend left] node[below, align=center] {$(B, 1)$} (4);
	\draw[->] (2) to[bend left] node[below, align=center] {$(B, 1)$} (4);
	\draw[->] (2) to[bend right] node[below, align=center] {$(\lnot s \land \lnot\mathit{pr}, 0)$} (1);
	\end{tikzpicture}	
	\caption{\ZX{Revised Reward machine for traveling on priority roads. $s$: stop; $\lnot s$ not stop; $pr$: end in priority road; $\lnot pr$: end in normal road. Intiitively, $p_0$ is in priority road and $p_1$ is in normal road, $p_2$ is after stopping in normal roads (should stop for only one time unit, consecutive stopping also fails), $p_3$ fails and $p_4$ succeeds. }} \label{fig:ex:reward-machine}
\end{figure}

A corresponding labeled MDP is $\mdp = (\mdpStates, \mdpInit, \mdpActions, \mdpProb, \rmLabels, \rmLabelingFunction)$.
A state $s \in \mdpStates$ is a quintuple $(x, y, \mathit{tr}, \mathit{pStart}, \mathit{pEnd})$.
Coordinates $x$ and $y$ correspond to the physical location of the vehicle (on a discretized grid).
Boolean variable $\mathit{tr}$ denotes whether there is a traffic from the right.
Finally, Boolean variables $\mathit{pStart}$ and $\mathit{pEnd}$ denote whether a sign for a start (respectively, end) of the priority road is visible.

The set of actions is $\mdpActions = \set{(0,1), (0,-1), (1,0), (-1,0), (0,0)}$, corresponding to going north, south, west, east and staying in place.
The transition probability $\mdpProb$ is defined by 
\[ 
\mdpProb(s, a, s') = 
\begin{cases}
	0 &\neg (s \xrightarrow{a} s')\\
	0.7 &s \xrightarrow{a} s' \land (s'.x, s'.y) \in \mathcal{J} \land s'.\mathit{tr} = \top \\
	0.3 & s \xrightarrow{a} s' \land (s'.x, s'.y) \in \mathcal{J} \land s'.\mathit{tr} = \bot \\ 
	0.5 &s \xrightarrow{a} s' \land (s'.x, s'.y) \not\in \mathcal{J}\\
\end{cases}
\]
where $s \xrightarrow{a} s'$ defines possible transitions. 
More precisely,  $s \xrightarrow{a} s'\equiv (s.x, s.y) + a = (s'.x, s'.y) \land s'.\mathit{pStart} \Leftrightarrow (s'.x, s'.y) \in \mathit{PriorityStart} \land s'.\mathit{pEnd} \Leftrightarrow (s'.x, s'.y) \in \mathit{PriorityEnd}$, where \textit{PriorityStart} and \textit{PriorityEnd} are sets of locations containing signs for start and end of priority road.
The set of locations $\mathcal J$ represents an area for which there is expected increased traffic.
Note that the randomness comes from the the actions of other cars, so the same action can bring the care into a state with traffic and the one without traffic.

The set of labels is $\set{\mathit{tr}, \mathit{pr}, y, B}$ and the labeling function $\rmLabelingFunction$ is defined by
\begin{align*}
\mathit{tr} \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.\mathit{tr} = \top \\
\mathit{pr} \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.\mathit{pStart} = \top \\
&\lor(s.\mathit{pStart} = \top \land s'.\mathit{pEnd} = \bot )\\
y \in \rmLabelingFunction(s,a,s') &\Leftrightarrow a = (0,0)\\
B \in \rmLabelingFunction(s,a,s') &\Leftrightarrow s'.x = x_B \land s'.y = y_B
\end{align*}

==> belief_RM.tex <==

\section{Inference of Belief Reward Machine and Policies in RL for Stochastic Games with Incomplete Information}

The belief reward machine is a reward machine where the labels can be functions of (estimated) intentions of the agents (on different reasoning levels).

\begin{definition}%[Reward Mealy machines]
\label{def:rewardMealyMachines}
A \emph{reward machine} 
$\machine = (\mealyStates, \mealyInit, \mealyInputAlphabet, \mealyOutputAlphabet, \mealyTransition, \mealyOutput)$ consists of 
a finite, nonempty set $\mealyStates$ of states, 
an initial state $\mealyInit \in \mealyStates$, 
an input alphabet $\mealyInputAlphabet$,
an output alphabet $\mealyOutputAlphabet$, 
a (deterministic) transition function $\mealyTransition \colon \mealyStates \times \mealyInputAlphabet \to \mealyStates$, 
and an output function $\mealyOutput \colon \mealyStates \times \mealyInputAlphabet \to \mealyOutputAlphabet$.
We define the size of $\machine$, denoted as $|\machine|$, to be $|\mealyStates|$ (i.e., the cardinality of the set $\mealyStates$).
\end{definition}

==> car_example.tex <==
\section{Motivating Example}
\label{sec_example} % TODO: change this to {sec:example}

As a motivating example, let us consider an autonomous vehicle navigating a residential area, as sketched in Figure~\ref{fig:ex:road-map}.
As is common in many countries, some of the roads are priority roads.
While traveling on a priority road, a car has the right-of-way and does not need to stop at intersections.
%Typically, there exist special signs on every intersection on the priority roads and no special signs on the intersections on the normal roads. 
In the example of Figure~\ref{fig:ex:road-map}, the priority road is indicated by gray shading, whereas the other roads are normal roads.


	\begin{figure}
		\centering
		\includegraphics[scale=0.4]{traffic_game2.pdf}
		\caption{Map of a residential area} \label{fig:ex:road-map}
	\end{figure}

% \begin{figure}[th]
% 	\centering
% 	\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
% 	% Road
% 	\draw[double=white, double distance=5mm, line width=.5mm] (0, 0) -- (5.5, 0) (0, -2) -- (5.5, -2) (1.5, 1) -- (1.5, -3) (4, 1) -- (4, -3);
% 	\fill[gray!25] ([yshift=-2.5mm]0, 0) rectangle ([yshift=2.5mm]5.5, 0);
% % 	([yshift=-2.5mm]0, -2) rectangle ([yshift=2.5mm]5.5, -2)
% % 	\draw[->, thick] (2.5, -0.1)--(3, -0.1); 
% % 	\draw[->, thick] (3, 0.1)--(2.5, 0.1);

% % 	\draw[->, thick] (2.5, -2.1)--(3, -2.1);
% %     \draw[->, thick] (3, -1.9)--(2.5, -1.9);
    
% % 	\draw[->, thick] (1.4, -0.8)--(1.4, -1.3);  
% %     \draw[->, thick] (1.6, -1.3)--(1.6, -0.8);                                                                            

% % 	\draw[->, thick] (3.9, -0.8)--(3.9, -1.3);  
% %     \draw[->, thick] (4.1, -1.3)--(4.1, -0.8);        
	
% 	\node at (0.7, -0.1){\includegraphics[scale=0.02]{figures/car}};
	
% 	% Markings
% 	\draw[dashed] (0, 0) -- (5.5, 0) (0, -2) -- (5.5, -2);
% 	\draw[dashed] (1.5, 1) -- (1.5, .25) (4, 1) -- (4, .25) (1.5, -.25) -- (1.5, -1.75) (4, -.25) -- (4, -1.75) (1.5, -2.25) -- (1.5, -3) (4, -2.25) -- (4, -3);
	
% 	% Labels
% 	\node[font=\bfseries] at (0, -0.1) {A};
% 	\node[font=\bfseries] at (5.5, -2.1) {B};
	
% 	\end{tikzpicture}
	
% 	\caption{Map of a residential area.} \label{fig:ex:road-map}
% \end{figure}

Let us assume that the task of the ego vehicle is to drive from position ``A'' to position ``D'' to pick up a passenger there and then take the passenger to position ``B''. In the meantime, the task of the other vehicle is simply to drive from position ``B'' to position ``C''.
To simplify matters, we are here only interested in the traffic rules concerning the right-of-way and how the vehicle acts at intersections with respect to the traffic from the intersecting roads.
Moreover, we make the following two further simplifications: (1) the vehicle correctly senses whether it is on a priority road and (2) the vehicle always stays in the road and goes straight forward while not at the intersections. We also assume that if two roads intersect, then at most one of them is a priority road.                     

The vehicle is obeying the traffic rules if and only if
\begin{itemize}
	\item it is traveling on a priority road and does not stop at any intersection (as the intersecting road must be a normal road);
	\item it is traveling on a normal road and does not stop at the intersection if there is no traffic at the intersecting road (whether it is normal or priority road).
	\item it is traveling on a normal road and yield to the traffic on the intersecting road if the intersecting road is a priority road.
\end{itemize}

Note that the above traffic rules do not specify what a vehicle on the normal road should do if there is traffic on the normal intersecting road. Specifically, if a vehicle on a normal road is encountering another vehicle on an intersecting normal road, then the vehicle could either yield or not yield to the other vehicle. If one of the two vehicles on the normal roads yields to the other vehicle, then we say that both vehicles are performing desired behaviors; if both of them do not yield, it will cause a collision and we say that both vehicles are performing undesired behaviors; and if both of them yield to the other vehicle, then the two vehicles are stuck at the intersection and we also say that both vehicles are performing undesired behaviors.

% In particular, the vehicle violates the rules and does not get a reward if it yields on a priority road or on a normal road when there is no traffic on the intersecting road.


We intend to achieve the above task in the setting of episodic RL. 
Specifically, after each episode of 100 time units, 
the ego vehicle receives a reward of 1 if it reached ``B'' with the passenger while obeying the traffic rules and performing desired behaviors;
otherwise it receives a reward of 0. 
It can be seen that the (implicit) reward function is non-Markovian 
(the reward depends not only on the current state, but also on the history of states 
from which one can decide if the traffic rules were obeyed).

In the example, we consider the situation where the two vehicles will arrive at intersection 2 at the same time if both of them follow the traffic rules (as otherwise the two vehicles do not need to interact with each other and the game can be reduced to decoupled planning of the two vehicles).

\noindent\textbf{Alternative Scenario I:} If the ego agent reaches shop ``E'' before the other agent, then the ego agent can achieve a reward of 2 if it reaches ``F'' afterwards and it can achieve a reward of 1 if it reaches ``C'' afterwards; and if the ego agent reaches shop ``E'' after the other agent, then the ego agent can achieve a reward of 0 if it reaches ``F'' afterwards and it can achieve a reward of 1 if it reaches ``C'' afterwards. On the other hand, if the other agent reaches shop ``E'' before the ego agent, then the other agent can achieve a reward of 2 if it reaches ``F'' afterwards and it can achieve a reward of 1 if it reaches ``C'' afterwards; and if the other agent reaches shop ``E'' after the ego agent, then the other agent can achieve a reward of 0 if it reaches ``F'' afterwards and it can achieve a reward of 1 if it reaches ``C'' afterwards.


\noindent\textbf{Alternative Scenario II:} If the ego agent reaches shop ``E'' before the other agent, then the ego agent can achieve a reward of 3 if it then reaches ``F'' before the other agent, a reward of 2 if it then reaches ``F'' after the other agent, and a reward of 1 if it doesn't reach ``F'' but reaches ``C'' afterwards; and if the ego agent reaches shop ``E'' after the other agent, then the ego agent can achieve a reward of 0 if it reaches ``F'' afterwards and it can achieve a reward of 1 if it reaches ``C'' afterwards. On the other hand, if the other agent reaches shop ``E'' before the ego agent, then the other agent can achieve achieve a reward of 3 if it then reaches ``F'' before the ego agent, a reward of 2 if it then reaches ``F'' after the ego agent, and a reward of 1 if it doesn't reach ``F'' but reaches ``C'' afterwards; and if the other agent reaches shop ``E'' after the ego agent, then the other agent can achieve a reward of 1 if it reaches ``F'' before the ego agent and a reward of 0 if it reaches ``F'' after the ego agent and it can achieve a reward of 0 if it reaches ``C'' afterwards.


	\begin{figure}
		\centering
		\includegraphics[scale=0.4]{traffic_game_scenario2.pdf}
		\caption{Map of a residential area} \label{fig_robust}
	\end{figure}

==> introduction.bak.tex <==
\section{Introduction}
\label{sec:introduction}
% Jean-Raphaël
% TODO: get inspiration Icarte's paper (ICML
% - background on multiagent
% - motivations RM for stochastic game (motivational example)
% TODO: tell a unique story.
% 
% FOCUS: GIVEN reward machine
%
%

% \paragraph{multiplayer games} % no RL


% \paragraph{MARL} % TO COMMENT
% Many interactions between several agents can be modeled as non-cooperative games %, i.e., general sum games,
% where every agent learns their optimal strategy concurrently.
% %
% \emph{Stochastic games} (SG)~\cite{Solan2015SG} model the interactions between multiple agents that interact with a single environment.
% \emph{Multi-agent reinforcement learning} (MARL)~\cite{Buoniu2010MARL} is a framework for multiple agents to optimize their strategies by repeated interactions with the environment.
% For instance, Nash-Q learning~\cite{hu2003nash} is a MARL algorithm, for learning strategies that result in a Nash equilibrium in non-cooperative settings.
% MARL finds applications in a variety of domains such as robotics or distributed control.



In multi-agent systems, agents interact with each other and the behavior of each agent can affect the performance of other agents. \emph{Multi-agent reinforcement learning} (MARL)~\cite{Buoniu2010MARL} is a framework for multiple agents to optimize their strategies by repeatedly interacting with the environment in a multi-agent system. The interactions between agents in MARL problems can be modeled as a \emph{stochastic game} (SG), where each agent seeks to reach a Nash equilibrium. In a Nash equilibrium, agents have best-response strategies considering other agent's actions.



% add transitions

% \paragraph{reward machines for complex tasks} % TO COMMENT
In many complex multi-agent games, the rewards can depend on the history of events (i.e., the reward function is non-Markovian). One way of encoding a non-Markovian reward function is by using a type of Mealy machine named \emph{reward machines}~\cite{icarte2018}. In this paper, we focus on stochastic games where each agent intends to complete a complex task
which can be represented by a reward machine capturing the temporal structure of the reward function. 
%

% We use \emph{Stochastic games} (SG)~\cite{Solan2015SG} to model games where the outcome of agent' actions is probabilistic.
% , ... non-markovian \cite{Solan2015SG}.

% TALK ABOUT HIERARCHICAL STUFF?
% The goal of some stochastic games can be complex tasks with sparse rewards,
% where there exists high-level knowledge capturing the temporal structure of the reward function. % [cite].
%

% \dots

% \paragraph{motivational example} % TO COMMENT
We introduce a variant of the PAC-MAN game as a motivational example,
where two agents try to capture each other,
and the task completion is defined based on complex conditions
(Figure \ref{fig:ex-capture-idea}). 
% A motivational example for this work is a capture game where two agents try to capture each other, and need to be the last agent at home to do that (Figure \ref{fig:ex-capture-idea}).
%
Two agents \agent[Ego] and \agent[Adv] evolve in a grid-world by taking synchronous steps towards adjacent cells. % (including their current cell).
We also introduce two power bases \location[EgoHome] and \location[AdvHome] that are fixed locations. %, that influence the dynamic of the game when agents reach these locations.
% We track these encounters with logical propositions such as \signal[EgoAtHome], \signal[AdvAtHome], and \signal[EgoMeetAdv] that evaluate on the lower level dynamics, and that the high level reward rely on.
We track whether the two agents encounter logical propositions such as \signal[EgoAtHome], \signal[AdvAtHome], and \signal[EgoMeetAdv] or not to evaluate the lower level dynamics and specify the high level reward.
For instance, the proposition \signal[EgoAtHome] is true when agent \agent[Ego] is at power base \location[EgoHome].
Similarly, the proposition \signal[EgoMeetAdv] is true when agents \agent[Ego] and \agent[Adv] meet on the same cell.
In the simplest variant of the game, the goal of each agent is to first reach its own power base and then capture the other agent. Each agent obtains a reward of 1 when its task is completed.
%but before doing that, he needs to be the last agent to visit its base
% during an encounter, the winner is the agent that visited the power base of its own color the most recently (as depicted by Figure \ref{fig:ex-capture-idea}).
Whenever agent \agent[Ego] arrives at its power base \location[EgoHome], agent \agent[Ego] becomes more powerful than agent \agent[Adv].
However, if agent \agent[Adv] then arrives at its power base \location[AdvHome], agent \agent[Adv] becomes the more powerful agent.
% The most powerful agent can capture the other.
The more powerful agent is capable to capture the other agent.
%(agent's base are fixed locations on the map, denoted by \location[EgoHome] and \location[AdvHome], that we suppose to be distinct).


% \paragraph{non-Markov games} % TO COMMENT
% A question arise: can the agents learn an reasonable strategy when the reward machine is unknown, i.e., can they outperform a memoryless strategy in a non-markov game?


% \paragraph{contrib} % TO COMMENT
% In this paper, we demonstrate that the prior knowledge of the reward machine enables the learning of the optimal strategy at a Nash equilibrium in a two-agent general-sum stochastic game with non-Markovian reward functions.
% % where the learning of a memoryless strategy would result in a suboptimal strategy.
% We develop an algorithm called Q-learning with Reward Machines for Stochastic Games (\algoName{}), where prior knowledge of the reward machine is given.
% We compare \algoName{} with common baselines such as Nash-Q learning~\cite{hu2003nash}.
% We compare \algoName{} with Nash Q-learning in augmented state space (Nash-QAS), where the learned strategy relies on the knowledge of current labels instead of a reward machine.
% We experimentally demonstrate that \algoName{} outperforms Nash-QAS.



In this paper, we address the challenge of learning complex tasks in two-agent general-sum stochastic games with non-Markovian reward functions. We develop an algorithm called Q-learning with Reward Machines for Stochastic Games ({\algoName{}}), where we use reward machines to specify the tasks and encode non-Markovian reward functions. 
% We demonstrate that the reward machines can enable task decomposition and task accomplishment for each agent.
In our proposed approach, we define the Q-function at a Nash equilibrium in augmented state space to adapt Q-learning to the setting of stochastic games when the tasks are specified by reward machines. 
During learning, at each time step, we formulate a stage game based on the current Q-functions in augmented state space and use the Lemke-Howson method to derive a Nash equilibrium. 
Q-functions in augmented state space are then updated according to the Nash-equilibrium. 
{\algoName{}} enables the learning of the best-response strategy at a Nash equilibrium for each agent. 
Q-functions learned in {\algoName{}} converge to the Q-functions at a Nash equilibrium if the stage game at each time step during learning has a global optimum point or a saddle point, and the agents update according to values at this point.
% where the learning of a memoryless strategy would result in a suboptimal strategy.
We test {\algoName{}} in three case studies and compare \algoName{} with common baselines such as Nash Q learning~\cite{hu2003nash} and Nash Q-learning in augmented state space. The results show that {\algoName{}} learns the best-response strategies at a Nash equilibrium effectively. 


\begin{figure}[ht] %fig:ex-capture-idea
    \centering
    
    \begin{subfigure}[t]{.40\linewidth}
        \centering
        \input{figs/intro-map.tikz}
        %\vspace{2em}
        \caption{
            Map of the environment.
            Agents \protect\agent[Ego] and \protect\agent[Adv] can move synchronously to an adjacent cell (or stay put) at each step.
            Locations \protect\location[EgoHome] and \protect\location[AdvHome] are called power bases.
        }
        \label{fig:ex-capture-idea:map}
    \end{subfigure}%
    \hspace*{0.03\linewidth}%
	\begin{subfigure}[t]{.56\linewidth}
        \centering
        % \input{figs/intro-rm-ego-sketch.tikz}
        % \caption{
        %     Sketch for a reward machine for agent \protect\agent[Ego]
        %     with sparse reward (zero when not specified on a transition).
        %     %The reward is sparse (zero when not specified on a transition).
        %     %We suppose that \protect\signal[EgoAtHome], \protect\signal[AdvAtHome] and \protect\signal[EgoMeetAdv] cannot all be true at the same time.
        %     %The game starts at the balanced state $\mealyCommonState_{bal}$, where no agent can capture the other.
        %     A proper reward machine would have to be deterministic.
        % }
        \input{figs/intro-rm-ego.tikz}
        \caption{
            Reward machine for agent \protect\agent[Ego]
            with sparse reward (zero when not specified on a transition).
            We suppose that \protect\signal[EgoAtHome], \protect\signal[AdvAtHome] and \protect\signal[EgoMeetAdv] cannot all be true at the same time.
            A proper reward machine would have to be deterministic.
        }
        \label{fig:ex-capture-idea:reward-machine}
    \end{subfigure}%
    %
    \caption{
        The simplest variant of the PAC-MAN game is a symmetric zero-sum game where two agents try to capture each other.
        % The agent that was the last at its own color location can capture the other agent.
        The agent that visited its own power base the most recently can capture the other agent.
        The low-level stochastic game plays out in a grid world (\subref{fig:ex-capture-idea:map}) and
        the high-level reward is captured by (\subref{fig:ex-capture-idea:reward-machine}).
        %This is a zero-sum game, hence the reward machine for player \protect\agent[Adv] has the same structure as (\subref{fig:ex-capture:reward-machine-idea}) but the rewards are negated.
    }
    \label{fig:ex-capture-idea}
    
\end{figure} %fig:ex-capture-idea

==> preliminaries_old2.tex <==
% !TEX root = main.tex
\section{Preliminaries}
\label{sec:preliminaries}
In this section we introduce necessary background on stochastic game, reinforcement learning, and reward machines.

\subsection{Stochastic Games and Reward Machines}

\begin{definition}
\label{def:mdp}
A \emph{two-player general-sum stochastic game} is a tuple
$\sg = (\sgStates, \sgInit, \sgActionsEgo, \sgActionsAdv, \sgProb, \sgRewardFunctionEgo, \sgRewardFunctionAdv, \rmLabels, \rmLabelingFunction)$
consisting of a finite state space $\sgStates$ (consisting of states $\sgCommonState=[\sgCommonStateEgo; \sgCommonStateAdv]$ where $\sgCommonStateEgo$ and $\sgCommonStateAdv$ are the substates of the ego agent and the other agent, respectively), $\sgInit\in\sgStates$ is the initial state,
$\sgActionsEgo$ and $\sgActionsAdv$ are the finite set of actions for the ego agent and the other agent, respectively,
and 
$\sgProb \colon \sgStates\times \sgActionsEgo \times\sgActionsAdv\times \sgStates \rightarrow [0,1]$ is the probabilistic transition function.
The reward functions $\sgRewardFunctionEgo: (\sgStates \times \sgActionsEgo\times\sgActionsAdv)^+ \times \sgStates \rightarrow \reals$ and $\sgRewardFunctionAdv: (\sgStates \times \sgActionsEgo\times\sgActionsAdv)^+ \times \sgStates \rightarrow \reals$ specify the payoffs to the ego agent and the other agent, respectively.
Finally, a finite set $\rmLabels$ of propositional variables, 
and a labeling function $\rmLabelingFunction: \sgStates\times \sgActionsEgo\times\sgActionsAdv\times \sgStates\rightarrow 2^\rmLabels$
determine the set of relevant high-level events. We define the size of $\sg$, denoted as $|\sg|$, to be $|\sgStates|$ (i.e., the cardinality of the set $\sgStates$).
\end{definition}

Our definition of the stochastic game differs from the ``usual'' definition used in reinforcement learning (e.g., \cite{sutton2018reinforcement}) in two ways.
First, the reward functions $\sgRewardFunction$ is defined over the whole history (i.e., the reward is \emph{non-Markovian}).
Second, Definition~\ref{def:mdp} includes a set $\rmLabels$ of propositions and a labeling function $\rmLabelingFunction$ assigning sets of propositions---also called \emph{labels}---to each transition $(s, a_e, a_a, s')$ of a stochastic game.
% Labels represent a high-level description of transitions, sufficient to express a reward.
Labels represent a high-level description of a transition that is sufficient to express a reward.
They represent expert knowledge of what is relevant for successfully executing a task and are assumed to be available to both the agent and the other agent.

% In the motivating example with the autonomous vehicle, for instance, it is enough to reason about the vehicle's behavior while entering an intersection from a priority or an normal road (and these would be the propositional variables).
% Note, however, that the full state space is still necessary to capture the model's dynamics, which might vary across different elements of $\sgStates$.



A \emph{trajectory} is
a sequence of states and actions $s_0 a_{e,0} a_{a,0} s_1 \ldots s_k a_{e,k}a_{a,k} s_{k+1}$,
with $s_0 = \sgInit$. 
Its corresponding \emph{label sequence} is $\sgLabel_0 \sgLabel_1\ldots \sgLabel_{k}$
where $\rmLabelingFunction(\sgCommonState_j, a_{e,j}, a_{a,j}, \sgCommonState_{j+1}) = \sgLabel_j$ for each $j \leq k$.
Similarly, the corresponding \emph{reward sequence} is $\sgRewards_1\ldots\sgRewards_k$,
where $\sgRewards_j = \sgRewardFunction(\trajectory{j})$, for each $j \leq k$. 
We call the pair $(\inputTrace, \outputTrace):=(\sgLabel_1\ldots\sgLabel_k, \sgRewards_1\ldots\sgRewards_k)$ a \emph{trace}.


For the ego agent and the other agent, they both observe the same trajectory $s_0 a_0 s_1 a_1 \ldots s_k a_k s_{k+1}$. The ego agent achieves a reward $r_e=\sum_{j=0}^{k} \sgDiscount^j \sgRewardFunctionEgo(s_0a_{e, 0}a_{a, 0}\ldots s_j a_{e, j} a_{a, j}s_{j+1})$, and the other agent achieves a reward $r_a=\sum_{j=0}^{k} \sgDiscount^j \sgRewardFunctionAdv(s_0a_{e, 0}a_{a, 0}\ldots s_j a_{e, j} a_{a, j}s_{j+1})$.

% now that gamma is in the definition, it is not necessary
%where $\sgDiscount \in [0,1)$ is a discount factor. 

% A \emph{behavior strategy} $\pi_e$ of the ego agent is a function mapping the trajectory in $\sgStates\times\sgActionsEgo\times\sgActionsAdv\times\dots\sgStates$ to a probability distribution over actions in $\sgActionsEgo$. A \emph{behavior strategy} $\pi_a$ of the other agent is a function mapping the trajectory in $\sgStates\times\sgActionsEgo\times\sgActionsAdv\times\dots\sgStates$ to a probability distribution over actions in $\sgActionsAdv$.
% At state $s\in \sgStates$, an ego agent using policy $\policy$ picks an action $a$ with probability $\policy(s, a)$,
% and the new state $s'$ is chosen with probability $\sgProb(s, a, s')$. 
% A policy $\policy$ and the initial state $\sgInit$ together determine a stochastic process and we write 
% $S_0 A_0 S_1 \ldots$ for the random trajectory of states and actions.

In reinforcement learning, the objective of the ego agent and the other agent is to maximize the expected cumulative reward $\displaystyle\mathbb{E}_{\pi_e}[r_e]$ and $\mathbb{E}_{\pi_a}[r_a]$, respectively.


%which depends only on the last transition
%(i.e., $\sgRewardFunction(\zeta\cdot(s,a)s') = \sgRewardFunction(\zeta'\cdot(s,a)s')$
%for all $\zeta, \zeta'\in (\sgStates\times\sgActions)^*$, where we use $\cdot$ to denote concatenation).

%Our definition of MDPs corresponds to the ``usual'' definition of MDPs (e.g., \cite{Puterman}),  
%except that we have introduced
%a set of high-level propositions (i.e., labels) $\rmLabels$ 
%and a labeling function $\rmLabelingFunction$ assigning sets of propositions (\emph{labels}) to each transition $(s, a, s')$ of an MDP. Besides, the definition of the reward function assumes that the reward is a function of the whole trajectory, i.e., 
%the reward is \emph{non-Markovian}.

%We use the labels to define (general) reward functions through \emph{reward machines}.
\zx{Modify this paragraph} Encoding a (non-Markovian) reward in a type of finite-state machine is achieved by reward machines~\cite{DBLP:conf/icml/IcarteKVM18,LTLAndBeyond}.
\footnote{
	The reward machines we are using are the so-called \emph{simple reward machines} in the parlance of~\cite{DBLP:conf/icml/IcarteKVM18},
	where every output symbol is a real number.
}
Technically, a reward machine is a special instance of a Mealy machine~\cite{DBLP:books/daglib/0025557},
the one that has real numbers as its output alphabet
and subsets of propositional variables (originating from an underlying MDP) as its input alphabet.
(To accentuate this connection
in the following definition, we explicitly mention
both the input alphabet $\mealyInputAlphabet$
and the output alphabet $\mealyOutputAlphabet$.)


\begin{definition}%[Reward Mealy machines]
\label{def:rewardMealyMachines}
A \emph{reward machine} 
$\machine = (\mealyStates, \mealyInit, \mealyInputAlphabet, \mealyOutputAlphabet, \mealyTransition, \mealyOutput)$ consists of 
a finite, nonempty set $\mealyStates$ of states, 
an initial state $\mealyInit \in \mealyStates$, 
an input alphabet $\mealyInputAlphabet$,
an output alphabet $\mealyOutputAlphabet$, 
a (deterministic) transition function $\mealyTransition \colon \mealyStates \times \mealyInputAlphabet \to \mealyStates$, 
and an output function $\mealyOutput \colon \mealyStates \times \mealyInputAlphabet \to \mealyOutputAlphabet$.
We define the size of $\machine$, denoted as $|\machine|$, to be $|\mealyStates|$ (i.e., the cardinality of the set $\mealyStates$).
\end{definition}

% When a reward machine is in one of its finitely many states, 
% upon reading a label, 
% it outputs a reward and transitions into a next state. 
% Formally, the run of a reward machine $\machine$ on a sequence of labels $\sgLabel_1\ldots \sgLabel_k\in (\mealyInputAlphabet)^*$ is a sequence 
% $\mealyCommonState_0 (\sgLabel_1, \sgRewards_1) \mealyCommonState_1 (\sgLabel_2, \sgRewards_2)\ldots (\sgLabel_k, \sgRewards_k) \mealyCommonState_{k+1}$ of states and label-reward pairs such that $\mealyCommonState_0 = \mealyInit$
% and for all $i\in\set{0,\ldots, k}$, we have $\mealyTransition(\mealyCommonState_i, \sgLabel_i) = \mealyCommonState_{i+1}$ and $\mealyOutput(\mealyCommonState_i,\sgLabel_i) = \sgRewards_i$.
% We write $\machine(\sgLabel_1\ldots\sgLabel_k) = \sgRewards_1\ldots\sgRewards_k$ 
% to connect the input label sequence 
% %$\sgLabel_1\ldots\sgLabel_k$
% to the sequence of rewards
% %$\sgRewards_1\ldots\sgRewards_k$ 
% produced by the machine $\machine$.
% We say that
% a reward machine $\machine$ \emph{\implement s} 
% the reward function $\sgRewardFunction$ of an MDP
% if for every trajectory $\trajectory{k}$
% and the corresponding label sequence $\sgLabel_1\ldots \sgLabel_k$, 
% %the value of the reward function is captured by the last element of the reward sequence,
% %$\sgRewardFunction(\trajectory{k}) = \sgRewards_k$.
% the reward sequence equals $\machine(\sgLabel_1\ldots \sgLabel_k)$.
% \footnote{In general, there can be multiple reward machines that encode the reward function of an MDP---reward machines may differ on a label sequence that does not correspond to any trajectory of an underlying MDP.}

% %\RM{omit?}
% An interesting (and practically relevant) subclass of reward machines is given by Mealy machines with a specially marked subset of \emph{final states}, the output alphabet $\set{0, 1}$, and the output function mapping a transition to 1 if and only if the end-state is a final state and the transition is not a self-loop. 
% Additionally, final states must not be a part of any cycle, except for a self-loop.
% This special case can be used in reinforcement learning scenarios with \textit{sparse} reward
% functions (e.g., see the reward machines used in the case studies in \cite{DBLP:conf/icml/IcarteKVM18}). 

% \begin{figure}[t]
% 	\centering
% 	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
% 	\node[state,initial] (0) at (-0.5, 0) {$\mealyCommonState_0$};
% 	\node[state] (1) at (2.5, 0) {$\mealyCommonState_1$};
% 	\node[state] (2) at (5.5, 0) {$\mealyCommonState_2$};
% 	\node[state] (3) at (8.5, 0) {$\mealyCommonState_3$};	
% 	\node[state] (4) at (5.5, 4) {$\mealyCommonState_4$};
% 	\node[state, accepting] (5) at (11.5, 0){$\mealyCommonState_5$};
% 	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
% 	\draw[->] (0) to[left] node[above, align=center] {$(\lnot s_e \land \lnot p_e, 0)$} (1);
% 	% \node[] at  (0.8,0.1) {$Low$};
% % 	\draw[->] (0) to[loop below] node[align=center] {$(\lnot s \land p, 0)$} ();
% 	\draw[->] (1) to[right] node[above, align=center] {$(\textrm{D}_e, 0)$} (2);
% 	\draw[->] (3) to[bend right=60] node[sloped, above, align=center] {$(s_e, 0)$} (4);
% 	\draw[->] (2) to[bend right=60] node[above, align=center] {$(s_e\wedge\lnot s_a, 0)$} (3);
% 	\draw[->] (2) to[bend left=60] node[above, align=center] {$(s_a\wedge\lnot s_e, 0)$} (3);
% 	\draw[->] (0) to[bend left=60] node[right, align=center] {$(s_e, 0)$} (4);
% 	\draw[->] (1) to[bend left=60] node[left, align=center] {$(s_e, 0)$} (4);
% 	%	\draw[->] (1) to[bend left] node[above, align=center] {$(\lnot s \land \lnot p, 0)$} (3);
% 	\draw[->] (3) to[right] node[above, align=center] {$(\textrm{B}_e, 1)$} (5);
% 	\draw[->] (2) to[bend right] node[right, align=center] {$(s_e\wedge s_a, 0)$} (4);
% 	\draw[->] (2) to[bend left] node[left, align=center] {$(\lnot s_e \land \lnot s_a, 0)$} (4);
% 	\end{tikzpicture}	
% 	\caption{Reward machine for the ego vehicle. $s_e$: stops at an intersection; $p_e$: ends up on a priority road. An edge $(\lnot s_e \land \lnot p_e, 0)$ between $v_0$ and $v_1$ means that the reward machine will transition from $\mealyCommonState_0$ to $\mealyCommonState_1$ if the propositional formula $\lnot s_e \land \lnot p_e$ is true for a sensed label and it will output a reward equal to zero. } 
% 	\label{fig:ex:reward-machine}
% \end{figure}
 
% \begin{figure}[t]
% 	\centering
% 	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
% 	\node[state,initial] (0) at (-0.5, 0) {$\mealyCommonState_0$};
% 	\node[state] (1) at (2.5, 0) {$\mealyCommonState_1$};
% 	\node[state] (2) at (2.5, 4) {$\mealyCommonState_2$};
% 	\node[state, accepting] (3) at (5, 0){$\mealyCommonState_5$};
% 	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
% 	\draw[->] (0) to[bend right=60] node[below, align=center] {$(s_a\wedge\lnot s_a, 0)$} (1);
% 	\draw[->] (0) to[bend left=60] node[below, align=center] {$(s_a\wedge\lnot s_e, 0)$} (1);
% 	\draw[->] (1) to[bend right] node[right, align=center] {$(s_e\wedge s_a, 0)$} (2);
% 	\draw[->] (1) to[bend left] node[left, align=center] {$(\lnot s_e \land \lnot s_a, 0)$} (2);
% 	\draw[->] (1) to[right] node[above, align=center] {$(\textrm{C}_a, 0)$} (3);
% 	\draw[->] (0) to[bend left=60] node[right, align=center] {$(s_e, 0)$} (2);
% 	\end{tikzpicture}	
% 	\caption{Reward machine for the other vehicle. $s_a$: stops at an intersection; $p_a$: ends up on a priority road. } 
% 	\label{fig:ex:reward-machine-adv}
% \end{figure}

% Figure~\ref{fig:ex:reward-machine} shows a reward machine for our motivating example, where transitions not shown in the figure are self-loops with reward 0.
% Intuitively, state $\mealyCommonState_0$ corresponds to the ego vehicle traveling on a priority road, $\mealyCommonState_1$ corresponds to the ego vehicle traveling on the normal road, and $\mealyCommonState_2$ corresponds to the ego vehicle reaching D for picking up the passenger.
% While in states $\mealyCommonState_0$ or $\mealyCommonState_1$, the vehicle ends up in a sink state $\mealyCommonState_4$ 
% %(representing violation of the traffic rules) 
% if it stops at an intersection (labels for which the propositional formula $s_e$ is true).
% While in state $\mealyCommonState_2$, the ego vehicle gets to state $\mealyCommonState_3$ if either vehicle yields to the other vehicle ($(s_a\wedge\lnot s_e)\vee(\lnot s_a\wedge  s_e)$), and the ego vehicle gets to the sink state $\mealyCommonState_4$ if both vehicles do not yield ($\lnot s_a\wedge\lnot  s_e$) or both vehicles yield at the intersection ($s_a\wedge s_e$). 
% Finally, a reward of 1 is obtained the goal position B is reached.


%\begin{figure}[th]
%	\centering
%	\begin{tikzpicture}
%	\node[state] (0) at (0, 0) {$p_0$};
%	\node[state] (1) at (3.5, 0) {$p_1$};
%	\node[state] (x) at (0, - 3.5) {$p_x$};
%	\node[state] (2) at (4.5, - 3.5) {$p_2$};
%	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
%	\draw[->] (0) to[bend right] node[sloped, below, align=center] {$(\lnot B \land \mathit{tr} \land \lnot y, 0)$ \\ $(\lnot B \land \lnot \mathit{tr} \land y$,0)} (x);
%	\draw[->] (0) to[loop above] node[align=center] {$(\lnot B \land \lnot\textit{pr}, 0)$\\$(\lnot B \land \textit{tr} \land \mathit{y}, 0)$ \\ $(\lnot B \land \lnot\textit{tr} \land \lnot\mathit{y}, 0)$} ();
%	\draw[->] (0) to[bend right=10] node[sloped, above, align=center] {$(B, 1)$} (2);
%	\draw[->] (0) to[bend left=20] node {$(\lnot B \land \mathit{pr}, 0)$} (1);			
%	\draw[->] (1) to[loop above] node[align=center] {$(\lnot B \land \lnot\mathit{y}, 0)$ \\ $(\lnot B \land\mathit{pr}, 0)$} ();
%	\draw[->] (1) to[bend left] node [above]{$(\lnot B \land\lnot\mathit{pr}, 0)$} (0);
%	\draw[->] (1) to[bend left=20] node[align=left, sloped, below] {$(y,0)$} (x);
%	\draw[->] (1) to[bend left=10] node[align=center, sloped] {$(B, 1)$} (2);
%	\draw[->] (x) to[loop below] node {$(*,0)$} ();
%	\draw[->] (2) to[loop below] node {$(*,0)$} ();
%	\end{tikzpicture}	
%	\caption{Reward machine for traveling on priority roads} \label{fig:ex:reward-machine}
%\end{figure}
 


% \begin{algorithm}[t] 
% 	\DontPrintSemicolon
% 	\SetKwBlock{Begin}{function}{end function}       
% 	{ \textbf{Hyperparameter}: episode length \textit{eplength}, learning rate $\alpha$, discount factor $\gamma$ } \;
% 	{ \textbf{Input:} a reward machine $(\mealyStates, \mealyInit, \mealyInputAlphabet, \mealyOutputAlphabet, \mealyTransition, \mealyOutput)$, 
% 		a set of q-functions $\setOfQFunctions = \set{\qValue^{\mealyCommonState} | \mealyCommonState \in \mealyStates }$ }\;
% 	$\sgCommonState \gets \mathit{InitialState()}; \mealyCommonState \gets \mealyInit; \inputTrace \gets [ ]; \outputTrace \gets [ ]$ \;
% 	\For{$0 \leq t < \mathit{eplength}$ \label{algLine:taskLoopStart}} 
% 	{ { $\sgCommonAction \gets \text{GetEpsilonGreedyAction}(\qValue^{\mealyCommonState}, \sgCommonState)$ \label{algLine:choiceOfAction} } \;
% 		{ $\sgCommonState' \gets \text{ExecuteAction}(\sgCommonState, \sgCommonAction)$ } \;
% 		{  $\mealyCommonState' \gets \mealyTransition( \mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState') )$ \label{algLine:RMTransition} } \;
% 		{$\sgRewards \gets \mealyOutput(\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ \,   \remind{or observe reward in \algoName}\label{algLine:Reward}}  \;
% 		{ $\textcolor{black}{\qValue^{\mealyCommonState}(\sgCommonState, \sgCommonAction)\gets(1-\alpha)\qValue^{\mealyCommonState}(\sgCommonState, \sgCommonAction)+\alpha(\sgRewards+\gamma\max\limits_{\sgCommonAction}\qValue^{\mealyCommonState}(\sgCommonState', \sgCommonAction))}$ \label{algLine:update} }
% 		\For{$\hat{\mealyCommonState} \in \mealyStates \setminus \set{\mealyCommonState}$  \label{algLine:learningLoopStart}  } 
% 		{ 
% 			{ $\hat\mealyCommonState' \gets \mealyTransition(\hat\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ }  \;
% 			{ $\hat{\sgRewards} \gets \mealyOutput(\hat\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ } \;
% 			{ $\text{update }\qValue^{\hat\mealyCommonState}(\sgCommonState, \sgCommonAction) \text{ using reward }\hat{\sgRewards}$ \label{algLine:learningLoopEnd}} \; 
% 			}
% 		%{ $\inputTrace \gets \inputTrace\frown \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'); \outputTrace  \gets \outputTrace \frown\sgRewards$ \label{algLine:tracesConcatenation} } \;
% 		{ append  $\rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState')$ to $\inputTrace$; append $\sgRewards$ to $\outputTrace$ \label{algLine:tracesConcatenation}} \;
% 		{ $\sgCommonState \gets \sgCommonState'; \mealyCommonState \gets \mealyCommonState'$ \label{algLine:taskLoopEnd}} \;
% 	}
% 	{ \Return $(\inputTrace, \outputTrace, \setOfQFunctions)$ }
% 	\caption{QRM\_episode}
% 	\label{alg:QRMepisode}
% \end{algorithm}	


% \subsection{Reinforcement Learning With Reward Machines}


% In reinforcement learning, an agent explores the environment modeled by an MDP,
% receiving occasional rewards according to the underlying reward function \cite{sutton2018reinforcement}.
% One way to learn an optimal policy is tabular q-learning \cite{Watkins1992}.
% There, the value of the function $q(s,a)$, 
% which represents the expected future reward
% for the agent taking action $a$ in state $s$,
% is iteratively updated.
% For MDPs with a Markovian reward function, q-learning converges to an optimal policy in the limit provided that all state-action pairs are seen infinitely often~\cite{Watkins1992}.

% The QRM algorithm modifies q-learning to learn an optimal policy when the general reward function is encoded by a reward machine
% \cite{DBLP:conf/icml/IcarteKVM18}.
% Algorithm~\ref{alg:QRMepisode} shows one episode of the QRM algorithm
% (with episode length \textit{eplength}, learning rate $\alpha$, and discount factor $\gamma$ as its hyperparameters and a reward machine as its input).
% It maintains a set $\setOfQFunctions$ of q-functions, denoted as $\qValue^{\mealyCommonState}$ for each state $\mealyCommonState$ of the reward machine 
% (their initial values can be specified as an input to the algorithm).

% The current state $\mealyCommonState$ of the reward machine guides the exploration by determining which q-function is used to choose the next action (Line~\ref{algLine:choiceOfAction}).
% However, in each single exploration step, the q-functions corresponding to all reward machine states are updated (Lines~\ref{algLine:update} and \ref{algLine:learningLoopEnd}).


% %The exploration is guided by the information encoded in the reward machine (lines \ref{algLine:choiceOfAction} and~\ref{algLine:RMTransition}).
% %It consists of two nested parts: the task loop (lines \ref{algLine:taskLoopStart} to \ref{algLine:taskLoopEnd}) and 
% %the learning loop (lines \ref{algLine:learningLoopStart} to \ref{algLine:learningLoopEnd}).

% %The outer loop is similar to classical q-learning and explores the MDP for a horizon equal to the horizon length, $\mathit{eplength}$.
% %The exploration is guided by the information encoded in the reward machine (lines \ref{algLine:choiceOfAction} and~\ref{algLine:RMTransition}).
% %All $q$-functions receive their updates---the one corresponding to the current reward machine state of the agent, 
% %but also the ones corresponding to all the other states of the reward machine.

% The modeling hypothesis of QRM is that the rewards are known, but the transition probabilities are unknown. 
% When using QRM as a part of \algoName, this knowledge is not available and the rewards must be \emph{observed} (see Line~\ref{algLine:Reward}).
% During the execution of the episode, traces $(\inputTrace, \outputTrace)$ of the reward machine are collected (Line~\ref{algLine:tracesConcatenation}) and returned in the end.
% While not necessary for q-learning, the traces will be useful in our algorithm to check the consistency of an \textit{inferred} reward machine with rewards received from the environment.






==> preliminary_old.tex <==
% !TEX root = main.tex
\section{Preliminaries}
\label{sec:preliminaries}
In this section we introduce necessary background on reinforcement learning and reward machines.

\subsection{Stochastic Games and Reward Machines}

\begin{definition}
\label{def:mdp}
A \emph{labeled two-player stochastic game} is a tuple
$\sg = (\sgStates, \sgActionsEgo, \sgActionsAdv, \sgProb, \sgRewardFunctionEgo, \sgRewardFunctionAdv, \rmLabels, \rmLabelingFunction)$
consisting of a finite state space $\sgStates$ (consisting of states $\sgCommonState=[\sgCommonStateEgo; \sgCommonStateAdv]$ where $\sgCommonStateEgo$ and $\sgCommonStateAdv$ are the substates of the ego agent and the adversary, respectively), 
a finite set of actions $\sgActions$ (for both the ego agent and the adversary),
and a probabilistic transition function
$\sgProb \colon \sgStates\times \sgActions \times \sgStates \rightarrow [0,1]$.
The reward functions $\sgRewardFunctionEgo: (\sgStates \times \sgActions)^+ \times \sgStates \rightarrow \reals$ and $\sgRewardFunctionAdv: (\sgStates \times \sgActions)^+ \times \sgStates \rightarrow \reals$ specify the payoffs to the ego agent and the adversary, respectively.
Finally, a finite set $\rmLabels$ of propositional variables, 
and a labeling function $\rmLabelingFunction: \sgStates\times \sgActions\times \sgStates\rightarrow 2^\rmLabels$
determine the set of relevant high-level events. We define the size of $\sg$, denoted as $|\sg|$, to be $|\sgStates|$ (i.e., the cardinality of the set $\sgStates$).
\end{definition}

Our definition of the stochastic game differs from the ``usual'' definition used in reinforcement learning (e.g., \cite{sutton2018reinforcement}) in two ways.
First, the reward functions $\sgRewardFunction$ is defined over the whole history (i.e., the reward is \emph{non-Markovian}).
Second, Definition~\ref{def:mdp} includes a set $\rmLabels$ of propositions and a labeling function $\rmLabelingFunction$ assigning sets of propositions---also called \emph{labels}---to each transition $(s, a, s')$ of a stochastic game.
% Labels represent a high-level description of transitions, sufficient to express a reward.
Labels represent a high-level description of a transition that is sufficient to express a reward.
They represent expert knowledge of what is relevant for successfully executing a task and are assumed to be available to both the agent and the adversary.


% In the motivating example with the autonomous vehicle, for instance, it is enough to reason about the vehicle's behavior while entering an intersection from a priority or an ordinary road (and these would be the propositional variables).
% Note, however, that the full state space is still necessary to capture the model's dynamics, which might vary across different elements of $\sgStates$.

A \emph{policy} is a function mapping states in $\sgStates$ to a probability distribution over actions in $\sgActions$.
At state $s\in \sgStates$, an agent using policy $\policy$ picks an action $a$ with probability $\policy(s, a)$,
and the new state $s'$ is chosen with probability $\sgProb(s, a, s')$. 
A policy $\policy$ and the initial state $\sgInit$ together determine a stochastic process and we write 
$S_0 A_0 S_1 \ldots$ for the random trajectory of states and actions.

A \emph{trajectory} is a realization of this stochastic process:
a sequence of states and actions $s_0 a_0 s_1 \ldots s_k a_k s_{k+1}$,
with $s_0 = \sgInit$. 
Its corresponding \emph{label sequence} is $\sgLabel_0 \sgLabel_1\ldots \sgLabel_{k}$
where $\rmLabelingFunction(\sgCommonState_i, \sgCommonAction_{i}, \sgCommonState_{i+1}) = \sgLabel_i$ for each $i \leq k$.
Similarly, the corresponding \emph{reward sequence} is $\sgRewards_1\ldots\sgRewards_k$,
where $\sgRewards_i = \sgRewardFunction(\trajectory{i})$, for each $i \leq k$. 
We call the pair $(\inputTrace, \outputTrace):=(\sgLabel_1\ldots\sgLabel_k, \sgRewards_1\ldots\sgRewards_k)$ a \emph{trace}.


A trajectory $s_0 a_0 s_1 a_1 \ldots s_k a_k s_{k+1}$ achieves a reward $\sum_{i=0}^{k} \sgDiscount^i \sgRewardFunction(s_0a_0\ldots s_i a_i s_{i+1})$.
% now that gamma is in the definition, it is not necessary
%where $\sgDiscount \in [0,1)$ is a discount factor. 
In reinforcement learning, the objective of the agent is to maximize the expected cumulative reward, $\mathbb{E}_\policy[\sum_{i=0}^\infty \sgDiscount^i \sgRewardFunction(S_0A_0\ldots S_{i+1})]$.


%which depends only on the last transition
%(i.e., $\sgRewardFunction(\zeta\cdot(s,a)s') = \sgRewardFunction(\zeta'\cdot(s,a)s')$
%for all $\zeta, \zeta'\in (\sgStates\times\sgActions)^*$, where we use $\cdot$ to denote concatenation).

%Our definition of MDPs corresponds to the ``usual'' definition of MDPs (e.g., \cite{Puterman}),  
%except that we have introduced
%a set of high-level propositions (i.e., labels) $\rmLabels$ 
%and a labeling function $\rmLabelingFunction$ assigning sets of propositions (\emph{labels}) to each transition $(s, a, s')$ of an MDP. Besides, the definition of the reward function assumes that the reward is a function of the whole trajectory, i.e., 
%the reward is \emph{non-Markovian}.

%We use the labels to define (general) reward functions through \emph{reward machines}.
Encoding a (non-Markovian) reward in a type of finite-state machine is achieved by reward machines~\cite{DBLP:conf/icml/IcarteKVM18,LTLAndBeyond}.
\footnote{
	The reward machines we are using are the so-called \emph{simple reward machines} in the parlance of~\cite{DBLP:conf/icml/IcarteKVM18},
	where every output symbol is a real number.
}
Technically, a reward machine is a special instance of a Mealy machine~\cite{DBLP:books/daglib/0025557},
the one that has real numbers as its output alphabet
and subsets of propositional variables (originating from an underlying MDP) as its input alphabet.
(To accentuate this connection
in the following definition, we explicitly mention
both the input alphabet $\mealyInputAlphabet$
and the output alphabet $\mealyOutputAlphabet$.)


\begin{definition}%[Reward Mealy machines]
\label{def:rewardMealyMachines}
A \emph{reward machine} 
$\machine = (\mealyStates, \mealyInit, \mealyInputAlphabet, \mealyOutputAlphabet, \mealyTransition, \mealyOutput)$ consists of 
a finite, nonempty set $\mealyStates$ of states, 
an initial state $\mealyInit \in \mealyStates$, 
an input alphabet $\mealyInputAlphabet$,
an output alphabet $\mealyOutputAlphabet$, 
a (deterministic) transition function $\mealyTransition \colon \mealyStates \times \mealyInputAlphabet \to \mealyStates$, 
and an output function $\mealyOutput \colon \mealyStates \times \mealyInputAlphabet \to \mealyOutputAlphabet$.
We define the size of $\machine$, denoted as $|\machine|$, to be $|\mealyStates|$ (i.e., the cardinality of the set $\mealyStates$).
\end{definition}

When a reward machine is in one of its finitely many states, 
upon reading a label, 
it outputs a reward and transitions into a next state. 
Formally, the run of a reward machine $\machine$ on a sequence of labels $\sgLabel_1\ldots \sgLabel_k\in (\mealyInputAlphabet)^*$ is a sequence 
$\mealyCommonState_0 (\sgLabel_1, \sgRewards_1) \mealyCommonState_1 (\sgLabel_2, \sgRewards_2)\ldots (\sgLabel_k, \sgRewards_k) \mealyCommonState_{k+1}$ of states and label-reward pairs such that $\mealyCommonState_0 = \mealyInit$
and for all $i\in\set{0,\ldots, k}$, we have $\mealyTransition(\mealyCommonState_i, \sgLabel_i) = \mealyCommonState_{i+1}$ and $\mealyOutput(\mealyCommonState_i,\sgLabel_i) = \sgRewards_i$.
We write $\machine(\sgLabel_1\ldots\sgLabel_k) = \sgRewards_1\ldots\sgRewards_k$ 
to connect the input label sequence 
%$\sgLabel_1\ldots\sgLabel_k$
to the sequence of rewards
%$\sgRewards_1\ldots\sgRewards_k$ 
produced by the machine $\machine$.
We say that
a reward machine $\machine$ \emph{\implement s} 
the reward function $\sgRewardFunction$ of an MDP
if for every trajectory $\trajectory{k}$
and the corresponding label sequence $\sgLabel_1\ldots \sgLabel_k$, 
%the value of the reward function is captured by the last element of the reward sequence,
%$\sgRewardFunction(\trajectory{k}) = \sgRewards_k$.
the reward sequence equals $\machine(\sgLabel_1\ldots \sgLabel_k)$.
\footnote{In general, there can be multiple reward machines that encode the reward function of an MDP---reward machines may differ on a label sequence that does not correspond to any trajectory of an underlying MDP.}

%\RM{omit?}
An interesting (and practically relevant) subclass of reward machines is given by Mealy machines with a specially marked subset of \emph{final states}, the output alphabet $\set{0, 1}$, and the output function mapping a transition to 1 if and only if the end-state is a final state and the transition is not a self-loop. 
Additionally, final states must not be a part of any cycle, except for a self-loop.
This special case can be used in reinforcement learning scenarios with \textit{sparse} reward
functions (e.g., see the reward machines used in the case studies in \cite{DBLP:conf/icml/IcarteKVM18}). 
%\RM{end omit}
\begin{figure}[t]
	\centering
	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
	\node[state,initial] (0) at (-0.5, 0) {$\mealyCommonState_0$};
	\node[state] (1) at (2.5, 0) {$\mealyCommonState_1$};
	\node[state] (2) at (5.5, 0) {$\mealyCommonState_2$};
	\node[state] (3) at (2.5, 2) {$\mealyCommonState_3$};
	\node[state, accepting] (4) at (-1.5, 2) {$\mealyCommonState_4$};
	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
	\draw[->] (0) to[left] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	% \node[] at  (0.8,0.1) {$Low$};
	\draw[->] (0) to[loop below] node[align=center] {$(\lnot sp \land \mathit{pr}, 0)$} ();
	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(sp, 0)$} (2);
	\draw[->] (2) to[bend left=55] node[sloped, above, align=center] {$(\lnot sp \land \mathit{pr}, 0)$} (0);
	\draw[->] (2) to[bend right=60] node[left, align=center] {$(sp, 0)$} (3);
	\draw[->] (0) to[bend left=60] node[right, align=center] {$(sp, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$(\lnot sp, 0)$} (3);
	%	\draw[->] (1) to[bend left] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (3);
	\draw[->] (0) to[bend left] node[left, align=center] {$(\textrm{B}, 1)$} (4);
	% \draw[->] (1) to[bend left] node[below, align=center] {$(B, 1)$} (4);
	% \draw[->] (2) to[bend left] node[below, align=center] {$(B, 1)$} (4);
	\draw[->] (2) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	\end{tikzpicture}	
	\caption{Reward machine for the autonomous vehicle. $sp$: stops at an intersection; $pr$: ends up in a priority road. An edge $(\lnot \mathit{sp} \land \lnot \mathit{pr}, 0)$ between $v_0$ and $v_1$ means that the reward machine will transition from $\mealyCommonState_0$ to $\mealyCommonState_1$ if the propositional formula $\lnot \mathit{sp} \land \lnot \mathit{pr}$ is true for a sensed label and it will output a reward equal to zero. } 
	\label{fig:ex:reward-machine}
\end{figure}
 

Figure~\ref{fig:ex:reward-machine} shows a reward machine for our motivating example, where transitions not shown in the figure are self-loops with reward 0.
Intuitively, state $\mealyCommonState_0$ corresponds to the vehicle traveling on a priority road, while $\mealyCommonState_1$ and $\mealyCommonState_2$ correspond to the vehicle traveling and stopped on an ordinary road, respectively.
While in $\mealyCommonState_0$, the vehicle ends up in a sink state $\mealyCommonState_3$ 
%(representing violation of the traffic rules) 
if it stops at an intersection (labels for which the propositional formula $\mathit{sp}$ is true).
While in state $\mealyCommonState_1$, the vehicle gets to the sink state $\mealyCommonState_3$ if it does not stop at an intersection ($\lnot\mathit{sp}$), and gets to state $\mealyCommonState_2$ if it stops at an intersection ($\mathit{sp}$). 
While in state $\mealyCommonState_2$, the vehicle gets to the sink state $\mealyCommonState_3$ if it stops again at the same intersection ($\mathit{sp}$);
it gets back to state $\mealyCommonState_0$ if it enters a priority road ($\lnot \mathit{sp} \wedge \mathit{pr}$); 
and it gets back to state $\mealyCommonState_0$ if it keeps moving on an ordinary road ($\lnot \mathit{sp}\wedge \lnot \mathit{pr}$).
The reward machine switches among states $\mealyCommonState_0$, $\mealyCommonState_1$ and $\mealyCommonState_2$ if the vehicle is obeying the traffic rules.
Finally, a reward of 1 is obtained if from $\mealyCommonState_0$ the goal position B is reached.


%\begin{figure}[th]
%	\centering
%	\begin{tikzpicture}
%	\node[state] (0) at (0, 0) {$p_0$};
%	\node[state] (1) at (3.5, 0) {$p_1$};
%	\node[state] (x) at (0, - 3.5) {$p_x$};
%	\node[state] (2) at (4.5, - 3.5) {$p_2$};
%	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
%	\draw[->] (0) to[bend right] node[sloped, below, align=center] {$(\lnot B \land \mathit{tr} \land \lnot y, 0)$ \\ $(\lnot B \land \lnot \mathit{tr} \land y$,0)} (x);
%	\draw[->] (0) to[loop above] node[align=center] {$(\lnot B \land \lnot\textit{pr}, 0)$\\$(\lnot B \land \textit{tr} \land \mathit{y}, 0)$ \\ $(\lnot B \land \lnot\textit{tr} \land \lnot\mathit{y}, 0)$} ();
%	\draw[->] (0) to[bend right=10] node[sloped, above, align=center] {$(B, 1)$} (2);
%	\draw[->] (0) to[bend left=20] node {$(\lnot B \land \mathit{pr}, 0)$} (1);			
%	\draw[->] (1) to[loop above] node[align=center] {$(\lnot B \land \lnot\mathit{y}, 0)$ \\ $(\lnot B \land\mathit{pr}, 0)$} ();
%	\draw[->] (1) to[bend left] node [above]{$(\lnot B \land\lnot\mathit{pr}, 0)$} (0);
%	\draw[->] (1) to[bend left=20] node[align=left, sloped, below] {$(y,0)$} (x);
%	\draw[->] (1) to[bend left=10] node[align=center, sloped] {$(B, 1)$} (2);
%	\draw[->] (x) to[loop below] node {$(*,0)$} ();
%	\draw[->] (2) to[loop below] node {$(*,0)$} ();
%	\end{tikzpicture}	
%	\caption{Reward machine for traveling on priority roads} \label{fig:ex:reward-machine}
%\end{figure}
 


\begin{algorithm}[t] 
	\DontPrintSemicolon
	\SetKwBlock{Begin}{function}{end function}       
	{ \textbf{Hyperparameter}: episode length \textit{eplength}, learning rate $\alpha$, discount factor $\gamma$ } \;
	{ \textbf{Input:} a reward machine $(\mealyStates, \mealyInit, \mealyInputAlphabet, \mealyOutputAlphabet, \mealyTransition, \mealyOutput)$, 
		a set of q-functions $\setOfQFunctions = \set{\qValue^{\mealyCommonState} | \mealyCommonState \in \mealyStates }$ }\;
	$\sgCommonState \gets \mathit{InitialState()}; \mealyCommonState \gets \mealyInit; \inputTrace \gets [ ]; \outputTrace \gets [ ]$ \;
	\For{$0 \leq t < \mathit{eplength}$ \label{algLine:taskLoopStart}} 
	{ { $\sgCommonAction \gets \text{GetEpsilonGreedyAction}(\qValue^{\mealyCommonState}, \sgCommonState)$ \label{algLine:choiceOfAction} } \;
		{ $\sgCommonState' \gets \text{ExecuteAction}(\sgCommonState, \sgCommonAction)$ } \;
		{  $\mealyCommonState' \gets \mealyTransition( \mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState') )$ \label{algLine:RMTransition} } \;
		{$\sgRewards \gets \mealyOutput(\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ \,   \remind{or observe reward in \algoName}\label{algLine:Reward}}  \;
		{ $\textcolor{black}{\qValue^{\mealyCommonState}(\sgCommonState, \sgCommonAction)\gets(1-\alpha)\qValue^{\mealyCommonState}(\sgCommonState, \sgCommonAction)+\alpha(\sgRewards+\gamma\max\limits_{\sgCommonAction}\qValue^{\mealyCommonState}(\sgCommonState', \sgCommonAction))}$ \label{algLine:update} }
		\For{$\hat{\mealyCommonState} \in \mealyStates \setminus \set{\mealyCommonState}$  \label{algLine:learningLoopStart}  } 
		{ 
			{ $\hat\mealyCommonState' \gets \mealyTransition(\hat\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ }  \;
			{ $\hat{\sgRewards} \gets \mealyOutput(\hat\mealyCommonState, \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'))$ } \;
			{ $\text{update }\qValue^{\hat\mealyCommonState}(\sgCommonState, \sgCommonAction) \text{ using reward }\hat{\sgRewards}$ \label{algLine:learningLoopEnd}} \; 
			}
		%{ $\inputTrace \gets \inputTrace\frown \rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState'); \outputTrace  \gets \outputTrace \frown\sgRewards$ \label{algLine:tracesConcatenation} } \;
		{ append  $\rmLabelingFunction(\sgCommonState, \sgCommonAction, \sgCommonState')$ to $\inputTrace$; append $\sgRewards$ to $\outputTrace$ \label{algLine:tracesConcatenation}} \;
		{ $\sgCommonState \gets \sgCommonState'; \mealyCommonState \gets \mealyCommonState'$ \label{algLine:taskLoopEnd}} \;
	}
	{ \Return $(\inputTrace, \outputTrace, \setOfQFunctions)$ }
	\caption{QRM\_episode}
	\label{alg:QRMepisode}
\end{algorithm}	


\subsection{Reinforcement Learning With Reward Machines}


In reinforcement learning, an agent explores the environment modeled by an MDP,
receiving occasional rewards according to the underlying reward function \cite{sutton2018reinforcement}.
One way to learn an optimal policy is tabular q-learning \cite{Watkins1992}.
There, the value of the function $q(s,a)$, 
which represents the expected future reward
for the agent taking action $a$ in state $s$,
is iteratively updated.
For MDPs with a Markovian reward function, q-learning converges to an optimal policy in the limit provided that all state-action pairs are seen infinitely often~\cite{Watkins1992}.

The QRM algorithm modifies q-learning to learn an optimal policy when the general reward function is encoded by a reward machine
\cite{DBLP:conf/icml/IcarteKVM18}.
Algorithm~\ref{alg:QRMepisode} shows one episode of the QRM algorithm
(with episode length \textit{eplength}, learning rate $\alpha$, and discount factor $\gamma$ as its hyperparameters and a reward machine as its input).
It maintains a set $\setOfQFunctions$ of q-functions, denoted as $\qValue^{\mealyCommonState}$ for each state $\mealyCommonState$ of the reward machine 
(their initial values can be specified as an input to the algorithm).

The current state $\mealyCommonState$ of the reward machine guides the exploration by determining which q-function is used to choose the next action (Line~\ref{algLine:choiceOfAction}).
However, in each single exploration step, the q-functions corresponding to all reward machine states are updated (Lines~\ref{algLine:update} and \ref{algLine:learningLoopEnd}).


%The exploration is guided by the information encoded in the reward machine (lines \ref{algLine:choiceOfAction} and~\ref{algLine:RMTransition}).
%It consists of two nested parts: the task loop (lines \ref{algLine:taskLoopStart} to \ref{algLine:taskLoopEnd}) and 
%the learning loop (lines \ref{algLine:learningLoopStart} to \ref{algLine:learningLoopEnd}).

%The outer loop is similar to classical q-learning and explores the MDP for a horizon equal to the horizon length, $\mathit{eplength}$.
%The exploration is guided by the information encoded in the reward machine (lines \ref{algLine:choiceOfAction} and~\ref{algLine:RMTransition}).
%All $q$-functions receive their updates---the one corresponding to the current reward machine state of the agent, 
%but also the ones corresponding to all the other states of the reward machine.

The modeling hypothesis of QRM is that the rewards are known, but the transition probabilities are unknown. 
When using QRM as a part of \algoName, this knowledge is not available and the rewards must be \emph{observed} (see Line~\ref{algLine:Reward}).
During the execution of the episode, traces $(\inputTrace, \outputTrace)$ of the reward machine are collected (Line~\ref{algLine:tracesConcatenation}) and returned in the end.
While not necessary for q-learning, the traces will be useful in our algorithm to check the consistency of an \textit{inferred} reward machine with rewards received from the environment.






==> rm.tex <==
\begin{figure}[t]
	\centering
	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
	\node[state,initial] (0) at (-1, 0) {$\mealyCommonState_0$};
	\node[state] (1) at (2.5, 0) {$\mealyCommonState_1$};
	\node[state] (2) at (5.5, 0) {$\mealyCommonState_2$};
	\node[state] (3) at (2.5, 2) {$\mealyCommonState_3$};
	\node[state] (4) at (2.5, -4) {$\mealyCommonState_4$};
    \node[state] (5) at (5.5, -4) {$\mealyCommonState_5$};
    \node[state] (6) at (-1, -4) {$\mealyCommonState_6$};
    \node[state, accepting] (7) at (2.5, -7) {$\mealyCommonState_7$};
	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
	\draw[->] (0) to[left] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	% \node[] at  (0.8,0.1) {$Low$};
	\draw[->] (0) to[loop below] node[align=center] {$(\lnot sp \land \mathit{pr}, 0)$} ();
	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(sp, 0)$} (2);
	\draw[->] (2) to[bend left=80] node[sloped, below, align=center] {$(\lnot sp \land \mathit{pr}, 0)$} (0);
	\draw[->] (2) to[bend right=60] node[right, align=center] {$(sp  \lor E_a, 0)$} (3);
	\draw[->] (0) to[bend left=60] node[left, align=center] {$(sp \lor E_a, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$(\lnot sp  \lor E_a, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$(E_e  \land \lnot E_a, 1)$} (4);
	\draw[->] (2) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
    \draw[->] (4) to[bend right] node[sloped, below, align=center] {$(sp, 0)$} (5);
    \draw[->] (5) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (4);
    \draw[->] (5) to[bend left=50] node[sloped, below, align=center] {$(\lnot sp \land \mathit{pr}, 0)$} (6);
    \draw[->] (6) to[left] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (4);
    \draw[->] (4) to[right] node[left, align=center] {$(F_e \land \lnot F_a, 1)$} (7);
    \draw[->] (5) to[bend right=90] node[right, align=center] {$(sp  \lor F_a, 0)$} (3);
    \draw[->] (6) to[bend left=90] node[left, align=center] {$(sp \lor F_a, 0)$} (3);
    % 4->3 not sp lor F_a
	\end{tikzpicture}	
	\caption{Reward machine for the ego agent (using traffic rules in JIRP). $sp$: stops at an intersection; $pr$: ends up in a priority road; $E_e$: the ego agent reaches shop E;  $E_a$: the adversarial agent reaches shop E; $F_e$: the ego agent reaches shop F;  $F_a$: the adversarial agent reaches shop F. }
	\label{fig:ex:reward-machine}
\end{figure}


\begin{figure}[t]
	\centering
	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
	\node[state,initial] (0) at (-1, 0) {$\mealyCommonState_0$};
	\node[state] (1) at (2.5, 0) {$\mealyCommonState_1$};
	\node[state] (2) at (5.5, 0) {$\mealyCommonState_2$};
	\node[state] (3) at (2.5, 2) {$\mealyCommonState_3$};
	\node[state, accepting] (4) at (2.5, -1.5) {$\mealyCommonState_4$};
	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
	\draw[->] (0) to[left] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	% \node[] at  (0.8,0.1) {$Low$};
	\draw[->] (0) to[loop below] node[align=center] {$(\lnot sp \land \mathit{pr}, 0)$} ();
	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(sp, 0)$} (2);
	\draw[->] (2) to[bend left=80] node[sloped, below, align=center] {$(\lnot sp \land \mathit{pr}, 0)$} (0);
	\draw[->] (2) to[bend right=60] node[right, align=center] {$(sp  \lor E_e \lor F_e, 0)$} (3);
	\draw[->] (0) to[bend left=60] node[left, align=center] {$(sp \lor E_e \lor F_e, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$(\lnot sp  \lor E_e \lor F_e, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$((E_a \lor F_a) \land (\lnot E_e \land \lnot F_e ), 1)$} (4);
	\draw[->] (2) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	\end{tikzpicture}	
	\caption{Reward machine for the adversarial agent (using traffic rules in JIRP). $sp$: stops at an intersection; $pr$: ends up in a priority road; $E_e$: the ego agent reaches shop E;  $E_a$: the adversarial agent reaches shop E; $F_e$: the ego agent reaches shop F;  $F_a$: the adversarial agent reaches shop F. }
	\label{fig:ex:reward-machine}
\end{figure}


%%%%% new traffic tule %%%%%%%

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
	\node[state,initial] (0) at (-1.5, 0) {$\mealyCommonState_0$};
	\node[state] (1) at (3.5, 0) {$\mealyCommonState_1$};
	\node[state] (2) at (8.5, 0) {$\mealyCommonState_2$};
	\node[state] (3) at (3.5, 3) {$\mealyCommonState_3$};
	\node[state, accepting] (4) at (3.5, -1.8) {$\mealyCommonState_4$};
	\draw[<-, shorten <=1pt] (0.west) -- +(-.4, 0);
	\draw[->] (0) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr},, 0)$} (1);
    \draw[->] (1) to[bend right] node[above, align=center] {$(\lnot T \land \lnot sp \land \mathit{pr}, 0)$} (0);
	\draw[->] (1) to[loop right] node[align=center] {$(\lnot T \land \lnot sp \land \lnot \mathit{pr}, 0)$} ();
	\draw[->] (0) to[loop below] node[align=center] {$(\lnot sp \land \mathit{pr}, 0)$} ();
	\draw[->] (1) to[bend right] node[sloped, below, align=center] {$(T \land sp, 0)$} (2);
	\draw[->] (2) to[bend left=80] node[sloped, below, align=center] {$(\lnot sp \land \mathit{pr}, 0)$} (0);
	\draw[->] (2) to[bend right=60] node[right, align=center] {$(sp  \lor E_a \lor F_a, 0)$} (3);
	\draw[->] (0) to[bend left=60] node[left, align=center] {$(sp \lor E_a \lor F_a, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$((\lnot T \land sp)  \lor E_a \lor F_a, 0)$} (3);
	\draw[->] (1) to[right] node[left, align=center] {$(E_e \lor F_e, 1)$} (4);
	\draw[->] (2) to[bend right] node[above, align=center] {$(\lnot sp \land \lnot\mathit{pr}, 0)$} (1);
	\end{tikzpicture}	
	\caption{Reward machine for the ego agent (new traffic rules in JIRP-game). $sp$: stops at an intersection; $pr$: ends up in a priority road; $E_e$: the ego agent reaches shop E;  $E_a$: the adversarial agent reaches shop E; $F_e$: the ego agent reaches shop F;  $F_a$: the adversarial agent reaches shop F; T: other agent is at the same intersection and tries to enter it.}
	\label{fig:ex:reward-machine}
\end{figure}
